HEMVIP: Human Evaluation of Multiple Videos in Parallel

In many research areas, for example motion and gesture generation, objective measures alone do not provide an accurate impression of key stimulus traits such as perceived quality or appropriateness. The gold standard is instead to evaluate these aspects through user studies, especially subjective evaluations of video stimuli. Common evaluation paradigms either present individual stimuli to be scored on Likert-type scales, or ask users to compare and rate videos in a pairwise fashion. However, the time and resources required for such evaluations scale poorly as the number of conditions to be compared increases. Building on standards used for evaluating the quality of multimedia codecs, this paper instead introduces a framework for granular rating of multiple comparable videos in parallel. This methodology essentially analyses all condition pairs at once. Our contributions are 1) a proposed framework, called HEMVIP, for parallel and granular evaluation of multiple video stimuli and 2) a validation study confirming that results obtained using the tool are in close agreement with results of prior studies using conventional multiple pairwise comparisons.

==> demographics_table.tex <==
% For the same table in the arXiv version, see the file appendix.tex
\begin{table*}
\vspace{-86.5mm}
\centering
\caption{Demographics for the four studies.}
\label{tab:demographics}
\begin{tabular}{@{}lcccc@{}}
\toprule 
\multicolumn{1}{l}{Demographic} & Q1 & Q2 & Q3 & Q4 \\ 
 \midrule
\multicolumn{1}{l}{Age} & \multicolumn{1}{c}{$34\pm12$} & \multicolumn{1}{c}{$28\pm9$} & \multicolumn{1}{c}{$31\pm11$} & \multicolumn{1}{c}{$29\pm10$} \tabularnewline


\multicolumn{1}{l}{Gender (F/M)} & \multicolumn{1}{c}{17/29} & \multicolumn{1}{c}{34/12} & \multicolumn{1}{c}{24/22} & \multicolumn{1}{c}{25/21} \tabularnewline

\multicolumn{1}{l}{Native English speakers} & \multicolumn{1}{c}{89\%} & \multicolumn{1}{c}{83\%} & \multicolumn{1}{c}{79\%} & \multicolumn{1}{c}{87\%} \tabularnewline

\multicolumn{1}{l}{Task difficulty\textsuperscript{1}} & \multicolumn{1}{c}{$3.4\pm1.2$} & \multicolumn{1}{c}{$3.6\pm1.2$} & \multicolumn{1}{c}{$3.8\pm1$} & \multicolumn{1}{c}{$3.7\pm1$} \tabularnewline

\multicolumn{1}{l}{Primary residency\textsuperscript{2}} & \multicolumn{1}{c}{1/1/39/5/0/0} & \multicolumn{1}{c}{1/2/35/5/2/1} & \multicolumn{1}{c}{2/2/34/7/1/0} & \multicolumn{1}{c}{2/1/28/14/1/0} 
\tabularnewline
\bottomrule
\multicolumn{5}{l}{\textsuperscript{1}Question: ``This task was really easy'' (1 being disagree and 5 agree)}
\tabularnewline
\multicolumn{5}{l}{\textsuperscript{2}Africa/Asia/Europe/North America/Oceania/South America}
\end{tabular}
% \vspace{-6mm}
\end{table*}

==> pairwise_table.tex <==
\begin{table*}[tp!]
\centering
\caption{System contrasts from user studies, with 95\% confidence intervals and Holm-Bonferroni corrected $p$-values from Clopper-Pearson (C-P) tests (preference ignoring ties) and pairwise $t$-tests (mean rating). $R$ stands for ``rating''. Daggers (\textdagger) mark non-significant differences. The ``Vs.\ \cite{kucherenko2020gesticulator}'' columns report whether or not the findings of significance agree with the C-P tests on data from \cite{kucherenko2020gesticulator} reported in the final two columns. Empty cells signify agreement, while $+$ (or $-$) mean that HEMVIP found (or did not find) the difference significant, in contrast to \cite{kucherenko2020gesticulator}.}
\label{tab:pairs}
%{\scriptsize%
\begin{tabular}{@{}ll|ccc|ccc|lc@{}}
\toprule
& $A{\to}B$ & $\mathbb{E}[R_B{-}R_A]$ & $p$-val. & Vs.\ \cite{kucherenko2020gesticulator} &  $\mathbb{P}(R_B{>}R_A)$ & $p$-val. & Vs.\ \cite{kucherenko2020gesticulator} &  $ \mathbb{P}(R_B{>}R_A)$ from \cite{kucherenko2020gesticulator} & $p$-val.   \\
\midrule
 & Full${\to}$NoAR  & ${-}$12.1$\pm$2.4  & <10\textsuperscript{${-}$20}\hphantom{\textsuperscript{\textdagger}}  &  & 27\%{}$\in$(22,32)  & <10\textsuperscript{${-}$20}\hphantom{\textsuperscript{\textdagger}}  &  & 23\%{}$\in$(19,28)  & <10\textsuperscript{${-}$25}\hphantom{\textsuperscript{\textdagger}} \tabularnewline
 & Full${\to}$NoPCA  & \hphantom{${-}$}10.7$\pm$1.9  & <10\textsuperscript{${-}$24}\hphantom{\textsuperscript{\textdagger}}  &  & 76\%{}$\in$(71,80)  & <10\textsuperscript{${-}$25}\hphantom{\textsuperscript{\textdagger}}  &  & 56\%{}$\in$(49,63)  & 0.050\hphantom{\textsuperscript{\textdagger}} \tabularnewline
 & Full${\to}$NoFiLM  & \hphantom{${-}$0}3.5$\pm$1.7  & <10\textsuperscript{${-}$3\hphantom{0}}\hphantom{\textsuperscript{\textdagger}}  &  & 58\%{}$\in$(52,63)  & 0.003\hphantom{\textsuperscript{\textdagger}}  &  & 57\%{}$\in$(50,64)  & 0.049\hphantom{\textsuperscript{\textdagger}} \tabularnewline
Q1 & Full${\to}$NoSpeech  & \hphantom{0}${-}$2.9$\pm$1.6  & <10\textsuperscript{${-}$3\hphantom{0}}\hphantom{\textsuperscript{\textdagger}}  &  & 43\%{}$\in$(37,48)  & 0.003\hphantom{\textsuperscript{\textdagger}}  &  & 34\%{}$\in$(28,42)  & <10\textsuperscript{${-}$4\hphantom{0}}\hphantom{\textsuperscript{\textdagger}} \tabularnewline
 & Full${\to}$NoText  & ${-}$11.4$\pm$1.6  & <10\textsuperscript{${-}$36}\hphantom{\textsuperscript{\textdagger}}  &  & 19\%{}$\in$(14,23)  & <10\textsuperscript{${-}$38}\hphantom{\textsuperscript{\textdagger}}  &  & 17\%{}$\in$(12,23)  & <10\textsuperscript{${-}$26}\hphantom{\textsuperscript{\textdagger}} \tabularnewline
 & Full${\to}$NoVel  & \hphantom{${-}$0}3.0$\pm$1.6  & <10\textsuperscript{${-}$3\hphantom{0}}\hphantom{\textsuperscript{\textdagger}}  &  & 60\%{}$\in$(54,65)  & <10\textsuperscript{${-}$3\hphantom{0}}\hphantom{\textsuperscript{\textdagger}}  &  & 59\%{}$\in$(52,66)  & 0.024\hphantom{\textsuperscript{\textdagger}} \tabularnewline
 & NoPCA${\to}$GT  & \hphantom{${-}$}40.5$\pm$1.9  & <10\textsuperscript{${-}$99}\hphantom{\textsuperscript{\textdagger}}  &  & 99\%{}$\in$(97,100)  & <10\textsuperscript{${-}$99}\hphantom{\textsuperscript{\textdagger}}  &  & 97\%{}$\in$(94,99)  & <10\textsuperscript{${-}$85}\hphantom{\textsuperscript{\textdagger}} \tabularnewline
\midrule 
 & Full${\to}$NoAR  & \hphantom{0}${-}$1.1$\pm$2.1  & 0.516\textsuperscript{\textdagger}  &  & 50\%{}$\in$(45,56)  & 0.846\textsuperscript{\textdagger}  &  & 49\%{}$\in$(43,55)  & 0.747\textsuperscript{\textdagger} \tabularnewline
 & Full${\to}$NoPCA  & \hphantom{${-}$}11.5$\pm$1.9  & <10\textsuperscript{${-}$27}\hphantom{\textsuperscript{\textdagger}}  &  & 75\%{}$\in$(70,79)  & <10\textsuperscript{${-}$23}\hphantom{\textsuperscript{\textdagger}}  &  & 69\%{}$\in$(63,75)  & <10\textsuperscript{${-}$10}\hphantom{\textsuperscript{\textdagger}} \tabularnewline
 & Full${\to}$NoFiLM  & \hphantom{${-}$0}2.6$\pm$1.7  & 0.006\hphantom{\textsuperscript{\textdagger}}  &  & 56\%{}$\in$(51,62)  & 0.042\hphantom{\textsuperscript{\textdagger}}  &  & 57\%{}$\in$(51,63)  & 0.039\hphantom{\textsuperscript{\textdagger}} \tabularnewline
Q2  & Full${\to}$NoSpeech  & \hphantom{0}${-}$2.9$\pm$1.7  & 0.002\hphantom{\textsuperscript{\textdagger}}  &  & 45\%{}$\in$(40,50)  & 0.119\textsuperscript{\textdagger}  & $-$ & 33\%{}$\in$(27,40)  & <10\textsuperscript{${-}$6\hphantom{0}}\hphantom{\textsuperscript{\textdagger}} \tabularnewline
 & Full${\to}$NoText  & ${-}$12.0$\pm$1.7  & <10\textsuperscript{${-}$37}\hphantom{\textsuperscript{\textdagger}}  &  & 23\%{}$\in$(19,28)  & <10\textsuperscript{${-}$27}\hphantom{\textsuperscript{\textdagger}}  &  & 10\%{}$\in$(\hphantom{0}7,15)  & <10\textsuperscript{${-}$49}\hphantom{\textsuperscript{\textdagger}} \tabularnewline
 & Full${\to}$NoVel  & \hphantom{${-}$0}1.0$\pm$1.7  & 0.516\textsuperscript{\textdagger}  &  & 52\%{}$\in$(47,58)  & 0.761\textsuperscript{\textdagger}  &  & 57\%{}$\in$(50,63)  & 0.067\textsuperscript{\textdagger} \tabularnewline
 & NoPCA${\to}$GT  & \hphantom{${-}$}36.6$\pm$2.3  & <10\textsuperscript{${-}$99}\hphantom{\textsuperscript{\textdagger}}  &  & 95\%{}$\in$(92,98)  & <10\textsuperscript{${-}$95}\hphantom{\textsuperscript{\textdagger}}  &  & 98\%{}$\in$(95,99)  & <10\textsuperscript{${-}$94}\hphantom{\textsuperscript{\textdagger}} \tabularnewline
\midrule
 & Full${\to}$NoAR  & \hphantom{0}${-}$1.2$\pm$2.0  & 0.217\textsuperscript{\textdagger}  &  & 49\%{}$\in$(44,55)  & 0.735\textsuperscript{\textdagger}  &  & 50\%{}$\in$(44,56)  & 0.869\textsuperscript{\textdagger} \tabularnewline
 & Full${\to}$NoPCA  & \hphantom{${-}$}12.0$\pm$1.8  & <10\textsuperscript{${-}$32}\hphantom{\textsuperscript{\textdagger}}  &  & 77\%{}$\in$(72,81)  & <10\textsuperscript{${-}$28}\hphantom{\textsuperscript{\textdagger}}  &  & 71\%{}$\in$(65,77)  & <10\textsuperscript{${-}$10}\hphantom{\textsuperscript{\textdagger}} \tabularnewline
 & Full${\to}$NoFiLM  & \hphantom{${-}$0}2.1$\pm$1.7  & 0.023\hphantom{\textsuperscript{\textdagger}}  &  & 58\%{}$\in$(53,64)  & 0.003\hphantom{\textsuperscript{\textdagger}}  &  & 60\%{}$\in$(53,66)  & 0.003\hphantom{\textsuperscript{\textdagger}} \tabularnewline
Q3 & Full${\to}$NoAudio  & \hphantom{0}${-}$2.2$\pm$1.6  & 0.016\hphantom{\textsuperscript{\textdagger}}  &  & 42\%{}$\in$(36,47)  & 0.003\hphantom{\textsuperscript{\textdagger}}  &  & 33\%{}$\in$(26,39)  & <10\textsuperscript{${-}$6\hphantom{0}}\hphantom{\textsuperscript{\textdagger}} \tabularnewline
 & Full${\to}$NoText  & ${-}$11.2$\pm$1.6  & <10\textsuperscript{${-}$35}\hphantom{\textsuperscript{\textdagger}}  &  & 22\%{}$\in$(17,26)  & <10\textsuperscript{${-}$31}\hphantom{\textsuperscript{\textdagger}}  &  & 11\%{}$\in$(7,15)  & <10\textsuperscript{${-}$44}\hphantom{\textsuperscript{\textdagger}} \tabularnewline
 & Full${\to}$NoVel  & \hphantom{${-}$0}2.6$\pm$1.7  & 0.007\hphantom{\textsuperscript{\textdagger}}  &  & 53\%{}$\in$(47,59)  & 0.459\textsuperscript{\textdagger}  & $-$ & 60\%{}$\in$(53,67)  & 0.006\hphantom{\textsuperscript{\textdagger}} \tabularnewline
 & NoPCA${\to}$GT  & \hphantom{${-}$}37.4$\pm$2.2  & <10\textsuperscript{${-}$99}\hphantom{\textsuperscript{\textdagger}}  &  & 96\%{}$\in$(94,98)  & <10\textsuperscript{${-}$99}\hphantom{\textsuperscript{\textdagger}}  &  & 98\%{}$\in$(96,100)  & <10\textsuperscript{${-}$95}\hphantom{\textsuperscript{\textdagger}} \tabularnewline
\midrule 
 & Full${\to}$NoAR  & \hphantom{0}${-}$4.6$\pm$2.1  & <10\textsuperscript{${-}$4\hphantom{0}}\hphantom{\textsuperscript{\textdagger}}  & $\mathbf{+}$ & 41\%{}$\in$(36,46)  & <10\textsuperscript{${-}$3\hphantom{0}}\hphantom{\textsuperscript{\textdagger}}  & $\mathbf{+}$ & 47\%{}$\in$(41,52)  & 0.197\textsuperscript{\textdagger} \tabularnewline
 & Full${\to}$NoPCA  & \hphantom{${-}$}10.0$\pm$2.0  & <10\textsuperscript{${-}$21}\hphantom{\textsuperscript{\textdagger}}  &  & 71\%{}$\in$(66,76)  & <10\textsuperscript{${-}$17}\hphantom{\textsuperscript{\textdagger}}  &  & 69\%{}$\in$(63,75)  & <10\textsuperscript{${-}$9\hphantom{0}}\hphantom{\textsuperscript{\textdagger}} \tabularnewline
 & Full${\to}$NoFiLM  & \hphantom{${-}$0}2.0$\pm$1.8  & 0.043\hphantom{\textsuperscript{\textdagger}}  &  & 55\%{}$\in$(50,61)  & 0.050\textsuperscript{\textdagger}  & $\mathbf{-}$ & 59\%{}$\in$(52,65)  & 0.008\hphantom{\textsuperscript{\textdagger}} \tabularnewline
Q4 & Full${\to}$NoAudio  & \hphantom{0}${-}$3.8$\pm$1.7  & <10\textsuperscript{${-}$4\hphantom{0}}\hphantom{\textsuperscript{\textdagger}}  &  & 38\%{}$\in$(33,43)  & <10\textsuperscript{${-}$5\hphantom{0}}\hphantom{\textsuperscript{\textdagger}}  &  & 33\%{}$\in$(27,40)  & <10\textsuperscript{${-}$7\hphantom{0}}\hphantom{\textsuperscript{\textdagger}} \tabularnewline
 & Full${\to}$NoText  & ${-}$12.0$\pm$1.6  & <10\textsuperscript{${-}$40}\hphantom{\textsuperscript{\textdagger}}  &  & 20\%{}$\in$(16,25)  & <10\textsuperscript{${-}$34}\hphantom{\textsuperscript{\textdagger}}  &  & 14\%{}$\in$(10,19)  & <10\textsuperscript{${-}$38}\hphantom{\textsuperscript{\textdagger}} \tabularnewline
 & Full${\to}$NoVel  & \hphantom{${-}$0}1.7$\pm$1.7  & 0.043\hphantom{\textsuperscript{\textdagger}}  &  & 51\%{}$\in$(46,57)  & 0.623\textsuperscript{\textdagger}  & $\mathbf{-}$ & 58\%{}$\in$(51,64)  & 0.026\hphantom{\textsuperscript{\textdagger}} \tabularnewline
 & NoPCA${\to}$GT  & \hphantom{${-}$}36.2$\pm$2.4  & <10\textsuperscript{${-}$99}\hphantom{\textsuperscript{\textdagger}}  &  & 94\%{}$\in$(91,97)  & <10\textsuperscript{${-}$89}\hphantom{\textsuperscript{\textdagger}}  &  & 96\%{}$\in$(93,98)  & <10\textsuperscript{${-}$83}\hphantom{\textsuperscript{\textdagger}} \tabularnewline
\bottomrule
\end{tabular}
%}
%\vspace{-6mm}
\end{table*}

==> pairwise_table_old.tex <==
\begin{table*}[t!]
\centering
\caption{System contrasts from user studies, with 95\% confidence intervals and Holm-Bonferroni corrected $p$-values from Clopper-Pearson (C-P) tests (preference ignoring ties) and pairwise $t$-tests (mean rating). $R$ stands for ``rating''. Daggers (\textdagger) mark non-significant differences. The ``Like \cite{kucherenko2020gesticulator}?'' columns report whether or not the findings of significance agree with the C-P tests on data from \cite{kucherenko2020gesticulator} reported in the final two columns.}
\label{tab:pairs}
%{\scriptsize%
\begin{tabular}{@{}ll|ccc|ccc|lc@{}}
\toprule
& $A{\to}B$ & $\mathbb{E}[R_B{-}R_A]$ & $p$-val. & Like \cite{kucherenko2020gesticulator}? &  $\mathbb{P}(R_B{>}R_A)$ & $p$-val. & Like \cite{kucherenko2020gesticulator}? &  $ \mathbb{P}(R_B{>}R_A)$ from \cite{kucherenko2020gesticulator} & $p$-val.   \\
\midrule
%\multirow{7}{*}{Q1} & Full${\to}$NoAR & 27\%{}$\in$(22,32) & <10\textsuperscript{${-}$20}\hphantom{\textsuperscript{\textdagger}} & ${-}$12.1$\pm$2.4 & <10\textsuperscript{${-}$20}\hphantom{\textsuperscript{\textdagger}} & & \\
%& Full${\to}$NoPCA & 76\%{}$\in$(71,80) & <10\textsuperscript{${-}$25}\hphantom{\textsuperscript{\textdagger}} & \hphantom{${-}$}10.7$\pm$1.9 & <10\textsuperscript{${-}$24}\hphantom{\textsuperscript{\textdagger}} & & \\
%& Full${\to}$NoFiLM & 58\%{}$\in$(52,63) & 0.003\hphantom{\textsuperscript{\textdagger}} & \hphantom{${-}$0}3.5$\pm$1.7 & <10\textsuperscript{${-}$3\hphantom{0}}\hphantom{\textsuperscript{\textdagger}} & & \\
%& Full${\to}$NoSpeech & 43\%{}$\in$(37,48) & 0.003\hphantom{\textsuperscript{\textdagger}} & \hphantom{0}${-}$2.9$\pm$1.6 & <10\textsuperscript{${-}$3\hphantom{0}}\hphantom{\textsuperscript{\textdagger}} & & \\
%& Full${\to}$NoText & 19\%{}$\in$(14,23) & <10\textsuperscript{${-}$38}\hphantom{\textsuperscript{\textdagger}} & ${-}$11.4$\pm$1.6 & <10\textsuperscript{${-}$36}\hphantom{\textsuperscript{\textdagger}} & & \\
%& Full${\to}$NoVel & 60\%{}$\in$(54,65) & <10\textsuperscript{${-}$3\hphantom{0}}\hphantom{\textsuperscript{\textdagger}} & \hphantom{${-}$0}3.0$\pm$1.6 & <10\textsuperscript{${-}$3\hphantom{0}}\hphantom{\textsuperscript{\textdagger}} & & \\
%& NoPCA${\to}$GT & 99\%{}$\in$(97,100) & <10\textsuperscript{${-}$99}\hphantom{\textsuperscript{\textdagger}} & \hphantom{${-}$}40.5$\pm$1.9 & <10\textsuperscript{${-}$99}\hphantom{\textsuperscript{\textdagger}} & & \\
%\midrule
\multirow{7}{*}{Q2} & Full${\to}$NoAR &  \hphantom{0}${-}$1.1$\pm$2.1 & 0.516\textsuperscript{\textdagger} & \cmark & 50\%{}$\in$(45,56) & 0.846\textsuperscript{\textdagger} & \cmark & 49\%{}$\in$(43,55) & 0.747\textsuperscript{\textdagger}     \\
& Full${\to}$NoPCA & \hphantom{${-}$}11.5$\pm$1.9 & <10\textsuperscript{${-}$27}\hphantom{\textsuperscript{\textdagger}} & \cmark & 75\%{}$\in$(70,79) & <10\textsuperscript{${-}$23}\hphantom{\textsuperscript{\textdagger}} & \cmark & 69\%{}$\in$(63,75) & <10\textsuperscript{${-}$10}\hphantom{\textsuperscript{\textdagger}}     \\
& Full${\to}$NoFiLM & \hphantom{${-}$0}2.6$\pm$1.7 & 0.006\hphantom{\textsuperscript{\textdagger}} & \cmark & 56\%{}$\in$(51,62) & 0.042\hphantom{\textsuperscript{\textdagger}} & \cmark &  57\%{}$\in$(51,63) & 0.039\hphantom{\textsuperscript{\textdagger}}     \\
& Full${\to}$NoAudio &  \hphantom{0}${-}$2.9$\pm$1.7 & 0.002\hphantom{\textsuperscript{\textdagger}} & \cmark & 45\%{}$\in$(40,50) & 0.119\textsuperscript{\textdagger} & \xmark & 33\%{}$\in$(27,40) & <10\textsuperscript{${-}$6\hphantom{0}}\hphantom{\textsuperscript{\textdagger}} \\
& Full${\to}$NoText &  ${-}$12.0$\pm$1.7 & <10\textsuperscript{${-}$37}\hphantom{\textsuperscript{\textdagger}} & \cmark & 23\%{}$\in$(19,28) & <10\textsuperscript{${-}$27}\hphantom{\textsuperscript{\textdagger}} & \cmark & 10\%{}$\in$(\hphantom{0}7,15) & <10\textsuperscript{${-}$49}\hphantom{\textsuperscript{\textdagger}}     \\
& Full${\to}$NoVel & \hphantom{${-}$0}1.0$\pm$1.7 & 0.516\textsuperscript{\textdagger} & \cmark & 52\%{}$\in$(47,58) & 0.761\textsuperscript{\textdagger} & \cmark & 57\%{}$\in$(50,63) & 0.067\textsuperscript{\textdagger}     \\
& NoPCA${\to}$GT &  \hphantom{${-}$}36.6$\pm$2.3 & <10\textsuperscript{${-}$99}\hphantom{\textsuperscript{\textdagger}} & \cmark & 95\%{}$\in$(92,98) & <10\textsuperscript{${-}$95}\hphantom{\textsuperscript{\textdagger}} & \cmark & 98\%{}$\in$(95,99) & <10\textsuperscript{${-}$94}\hphantom{\textsuperscript{\textdagger}} \\
\bottomrule
\end{tabular}
%}
%\vspace{-6mm}
\end{table*}

\iffalse

\begin{table}[t!]
\caption{}
\label{tab:validation}
\begin{tabular}{lll}
\toprule
Gesticulator               & Validation study          &  Same        \\
\midrule
Full = NoAR               & full = NoAR              & \cmark     \\
Full {\textless} NoPCA      & full {\textless} NoPCA     & \cmark     \\
Full = NoFILM             & full < NoFILM            & \xmark     \\
Full {\textgreater} NoAudio & full = NoAudio           & \xmark \\
Full {\textgreater} NoText  & full {\textgreater} NoText & \cmark     \\
Full = NoVel              & full = NoVel             & \cmark     \\
\midrule
NoPCA {\textless} GT & NoPCA {\textless} GT & \cmark \\
\bottomrule
\end{tabular}
\end{table}

\fi
